Unsupervised Expressive Rules Provide Explainability and Assist Human Experts Grasping New Domains

Approaching new data can be quite deterrent; you do not know how your categories of interest are realized in it, commonly, there is no labeled data at hand, and the performance of domain adaptation methods is unsatisfactory. Aiming to assist domain experts in their first steps into a new task over a new corpus, we present an unsupervised approach to reveal complex rules which cluster the unexplored corpus by its prominent categories (or facets). These rules are human-readable, thus providing an important ingredient which has become in short supply lately - explainability. Each rule provides an explanation for the commonality of all the texts it clusters together. We present an extensive evaluation of the usefulness of these rules in identifying target categories, as well as a user study which assesses their interpretability.

==> intro_prev.tex <==
\section{Introduction} \label{sec:intro}
Here it happens again. For a given text understanding task, we are facing a new dataset, which we barely know, and for which we do not have labeled data. Understanding the unexplored data, and collecting first insights from it, is always a slow process. 

This is exactly what happened to us with the new datasets of listening comprehension over argumentative content \cite{Mirkin-etal:2018,mirkin2018listening}. These are datasets of recordings of spoken speeches of debate over controversial topics. Each speech is provided with the textual output of an automatic speech recognition system, \emph{ASR}. The ASR output is noisy and sometimes hard to read. 

One option is domain adaptation, using an existing model which was trained on another dataset for this task. However, often it results in unsatisfying performance \cite{ziser2018pivot}.

Indeed, for the task of argumentative sentences detection in ASR output, we took the neural network described in \citet{BlendNet} and trained it on a huge labeled dataset of written text (see \S \ref{sec:eval}). While precision was not bad, considering the major differences between written and spoken language, recall was too low for practical usage. We had to think of another approach.

When facing a new task, with no labeled data, but with some expertise in the domain, a practical first step is to manually write rules. These rules would identify some of the texts in which the target category (argumentative sentences, in our case) is realized. With these seed examples experts can get a better understanding of the occurrences of the target category in the new corpus, and use them as the beginning of labeled examples, towards the goal of having enough labeled data in the new corpus to allow supervised learning.

However, how can a domain expert write rules for an unknown corpus which is considerably different in characteristics than previously known corpora?

\begin{table*}[t]
 \resizebox{\linewidth}{!}{
\begin{tabular}{@{}cclc@{}}
    no. & Category in Dataset & Sentences Matched & Rules  \\ 
    %-------------------------------------------------------%
    \cmidrule[\heavyrulewidth](l){1-4}    

    \begin{tabular}{@{}c@{}} 1 \\2\\3 \end{tabular} &
    \begin{tabular}{@{}c@{}} Arguments\\ in \asrd{} \end{tabular} &
     
    \begin{tabular}{@{}l@{}} so \textbf{first} let us \textbf{address} the question \\ 
    our \textbf{second argument} is about \\ 
    my \textbf{first overview} is \end{tabular} &
     
     \begin{tabular}{@{}c@{}} \as{hyponym of rank} $+$\\ \as{WordNet super class of communication}\end{tabular}  \\ 
    %-------------------------------------------------------% 
    \cmidrule[\lightrulewidth](l){1-4}
      
    \begin{tabular}{@{}c@{}} 4 \\5\\6 \end{tabular} &
    \begin{tabular}{@{}c@{}} Arguments\\ in \asrd{} \end{tabular} &   

    \begin{tabular}{@{}l@{}} \textbf{additionally I think} that sam is \textbf{confused}    \\
    \textbf{ultimately}, \textbf{we think} that it \textbf{limits} the \\
    \textbf{obviously}, \textbf{we acknowledge} it's \textbf{important} \end{tabular} &
    
    \begin{tabular}{@{}c@{}} \as{adverb} $+$ \as{personal pronoun} $+$ \\ \as{hyponym of think} $+$ \as{sentiment word} \end{tabular} \\
   
    %-------------------------------------------------------%
    \cmidrule[\lightrulewidth](l){1-4}
      
    \begin{tabular}{@{}c@{}} 7 \\8\\9 \end{tabular} &
    \begin{tabular}{@{}c@{}} Major claims\\ in students\\\stgur{} \end{tabular} &   
    
    \begin{tabular}{@{}l@{}}     
    \textbf{for example}, \textbf{employer} always prefer to\\
    \textbf{for instance}, several \textbf{teenagers} play games\\
     as a matter \textbf{of fact}, \textbf{women} have proved
     \end{tabular} &
    
    \begin{tabular}{@{}c@{}} \as{preposition} + \\ \as{hyponym of psychological feature} + \\ \as{hyponym of causal agent} \end{tabular} \\
    
     %-------------------------------------------------------%
    \cmidrule[\lightrulewidth](l){1-4}
      
    \begin{tabular}{@{}c@{}} 10 \\11\\12 \end{tabular} &
    \begin{tabular}{@{}c@{}} background info\\ in \holj{} \end{tabular} & 
    
    \begin{tabular}{@{}l@{}}     
     \\
     \\
      
     \end{tabular} &
    
    \begin{tabular}{@{}c@{}} \as{adverb} +  \as{personal pronoun} + \\ \as{WordNet super class of emotion} \end{tabular} \\
    
    %-------------------------------------------------------%
    \cmidrule[\lightrulewidth](l){1-4}
      
    \begin{tabular}{@{}c@{}} 13\\14\\15 \end{tabular} &
    \begin{tabular}{@{}c@{}} unfair clauses\\ in \tos{} \end{tabular} & 
    
    \begin{tabular}{@{}l@{}}     
     \\
     \\
      
     \end{tabular} &
    
    \begin{tabular}{@{}c@{}} \as{adverb} +  \as{personal pronoun} + \\ \as{WordNet super class of emotion} \end{tabular} \\
    
    \cmidrule[\heavyrulewidth](l){1-4}
\end{tabular}
}

\caption{Rules which generalize sentences belonging to a certain category (bold words are those matched by the rule). The various datasets and categories are described in Section \ref{sec:data}}.
\label{tab:pattern_exmples}
\vspace{-0.2cm}
\end{table*}


In this paper we present a method for generating such rules automatically, with no need of any labeled data. We show that the generated rules can reveal the common categories of the corpus, even though the method for generating them never got these categories as an input (this is the case when the experts themselves are yet to be aware of the existence of these categories).

To automatically identify rules we use \grasp{} \cite{grasp}. This supervised algorithm finds highly expressive rules, in the form of patterns, which capture the common structures of a category of interest. However, it demands a set of texts in which the target category appears and a set in which it does not. Since we do no have labeled data, we have developed \graspl{}, an unsupervised version of \grasp{}. 

Instead of labeled sets, \graspl{} takes a \textit{background} corpus and contrasts it with the new corpus, the \textit{foreground} corpus. By this, it reveals rules which capture sentences that are common in the foreground but not in the background. Such sentences are expected to be correlated with (at least some of) the unique categories in the foreground -- the new corpus. Examples of such rules are given in Table \ref{tab:pattern_exmples}.\esmod{I'll describe one rule to show that rules are human-readable.}

Naturally, rules generated in an unsupervised manner would be noisy. In addition, the rules revealed by \graspl{} capture a mixture of the categories that exist in the foreground corpus, not necessarily all of them are relevant for the task at hand. 

At this stage, subject matter experts get into the loop. As rules are human-readable, and each one provides an explanation for why it clusters sentences together, experts can identify the subset of rules which, together, best capture the sentences of their category of interest. Experts can also take ideas from the rules suggested by \graspl{}, manually edit rules to better fit their needs, merge elements from several rules into new rules, or improve their own manual rules with generalizations offered by the suggested rules. 

Our evaluation, over various dataset of different domains, shows that in the list of rules \graspl{} generates there are many rules which can be used to identify sentences belonging to the categories of these datasets. 

to conclude, \graspl{} unsupervised rules are not supposed to be used as a model for classifying a target category, but rather help experts significantly expedite the process of working on new data. Generating them does not require labeled data or deep understanding of the data and therefore can be the first thing to do.\es{should we mention here the small ASR test set we release, or leave it to the dataset section?}

 
%======= commented out =======================%

\begin{comment}
We do not have such sets for the indicators identification task. However, based on our second observation above, we can split each sentence in the dataset into two halves to obtain a set of sentence beginnings and a set of sentence endings. Since we expect indicators to be much more abundant in the first set, we use it as the positive set for \grasp{} learning, and the endings set as its negative set. 


We show that \graspl{} provides interesting insights into these new spoken language corpora. For instance, we quickly learn that instead of the indicator \emph{``argue that''}, which is common in written language to precede an argument \cite{levy14,grasp}, in spoken speeches a common indicator is \emph{``our first argument is''}.

We release the test set of ASR arg mining evaluation.

\grasp{} removing its major barrier to entry - the need for labeled data.

\end{comment}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
